Block-Wise Mixed-Precision Quantization: Enabling High Efficiency for Practical ReRAM-based DNN Accelerators

Resistive random access memory (ReRAM)-based processing-in-memory (PIM) architectures have demonstrated great potential to accelerate Deep Neural Network (DNN) training/inference. However, the computational accuracy of analog PIM is compromised due to the non-idealities, such as the conductance variation of ReRAM cells. The impact of these non-idealities worsens as the number of concurrently activated wordlines and bitlines increases. To guarantee computational accuracy, only a limited number of wordlines and bitlines of the crossbar array can be turned on concurrently, significantly reducing the achievable parallelism of the architecture. While the constraints on parallelism limit the efficiency of the accelerators, they also provide a new opportunity for fine-grained mixed-precision quantization. To enable efficient DNN inference on practical ReRAM-based accelerators, we propose an algorithm-architecture co-design framework called \underline{B}lock-\underline{W}ise mixed-precision \underline{Q}uantization (BWQ). At the algorithm level, BWQ-A introduces a mixed-precision quantization scheme at the block level, which achieves a high weight and activation compression ratio with negligible accuracy degradation. We also present the hardware architecture design BWQ-H, which leverages the low-bit-width models achieved by BWQ-A to perform high-efficiency DNN inference on ReRAM devices. BWQ-H also adopts a novel precision-aware weight mapping method to increase the ReRAM crossbar's throughput. Our evaluation demonstrates the effectiveness of BWQ, which achieves a 6.08x speedup and a 17.47x energy saving on average compared to existing ReRAM-based architectures.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> todo.tex <==
% \begin{table}[t]
%   \centering
%   \caption{Model Performance On CIFAR-10 Dataset}
%   % \small
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     % \multirow{2}{*}{\textbf{Model}} & \multirow{1}{*}{\textbf{\#Params of}} & \multirow{1}{*}{\textbf{Compression}} & \multirow{1}{*}{\textbf{Activation}} & \multirow{2}{*}{\textbf{Test Acc}} & \multirow{1}{*}{\textbf{Compression}} \\
%     %  & \textbf{Base Model}& \textbf{Method} & \textbf{Bit-width} & & \textbf{Ratio} \\
%     \multirow{2}{*}{{Model}} & \multirow{1}{*}{{Model}} & \multirow{2}{*}{{Method}} & \multirow{1}{*}{{Act.}} & \multirow{2}{*}{{Acc}} & \multirow{2}{*}{{Comp}} \\
%      & {Size}& & {Prec.} & &  \\
%     % & & & & \\
%     \hline \hline
%     \multirow{3}{*}{ResNet18} & \multirow{3}{*}{11.17M} & Baseline & 32 & 95.38\% & 1x \\
%     & & BSQ & 4 & 95.38\% & 26.05x \\
%     & & BWQ-A & 3 & 94.59\% & 56.46x \\
%     \hline
%     \multirow{3}{*}{ResNet34} & \multirow{3}{*}{21.28M} & Baseline & 32 & 95.61\% & 1x \\
%     & & BSQ & 4 & 94.66\% & 83.86x \\
%     & & BWQ-A & 4 & 94.73\% & 117.52x \\
%     \hline
%     \multirow{3}{*}{VGG16-BN} & \multirow{3}{*}{33.65M} & Baseline & 32 & 92.60\% & 1x \\
%     & & BSQ & 3 & 92.45\% & 26.59x \\
%     & & BWQ-A & 3 & 92.60\% & 136.01x \\
%     \hline
%     \multirow{3}{*}{VGG19-BN} & \multirow{3}{*}{38.96M} & Baseline & 32 & 92.94\% & 1x \\
%     & & BSQ & 3 & 92.84\% & 28.15x \\
%     & & BWQ-A & 3 & 91.96\% & 443.01x \\
%     \hline
%     \multirow{3}{*}{ResNet20} & \multirow{3}{*}{0.27M} & Baseline & 32 & 92.61\% & 1x \\
%     & & BSQ & 3 & 92.16\% & 13.76x \\
%     & & BWQ-A & 3 & 92.07\% & 16.04x \\
%     \hline
%     \multirow{3}{*}{MobileNetV2} & \multirow{3}{*}{2.30M} & Baseline & 32 & 94.43\% & 1x \\
%     & & BSQ & 4 & 94.24\% & 5.73x \\
%     & & BWQ-A & 3 & 93.54\% & 47.34x \\
%     \bottomrule
%   \end{tabular}
%   \label{cifar10}
%   % \vspace{-6pt}
% \end{table}




% \begin{table}
% % \vspace{-6pt}
%   \centering
%   \caption{Model Performance On CIFAR-100 Dataset}
%   % \small
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{2}{*}{{Model}} & \multirow{1}{*}{{Model}} & \multirow{2}{*}{{Method}} & \multirow{1}{*}{{Act.}} & \multirow{2}{*}{{Acc}} & \multirow{2}{*}{{Comp}} \\
%      & {Size}& & {Prec.} & &  \\
%     % & & & & \\
%     \hline \hline
%     \multirow{3}{*}{ResNet18} & \multirow{3}{*}{11.22M} & Baseline & 32 & 75.61\% & 1x \\
%     & & BSQ & 4 & 76.35\% & 6.21x \\
%     & & BWQ-A & 4 & 75.31\% & 45.97x \\
%     \hline
%     \multirow{3}{*}{ResNet34} & \multirow{3}{*}{21.33M} & Baseline & 32 & 76.41\% & 1x \\
%     & & BSQ & 4 & 76.37\% & 33.40x \\
%     & & BWQ-A & 4 & 76.16\% & 63.93x \\
%     \hline
%     \multirow{3}{*}{VGG16-BN} & \multirow{3}{*}{34.02M} & Baseline & 32 & 72.93\% & 1x \\
%     & & BSQ & 4 & 72.37\% & 19.88x \\
%     & & BWQ-A & 3 & 72.87\% & 50.42x \\
%     \hline
%     \multirow{3}{*}{VGG19-BN} & \multirow{3}{*}{39.33M} & Baseline & 32 & 72.94\% & 1x \\
%     & & BSQ & 4 & 72.05\% & 23.09x \\
%     & & BWQ-A & 3 & 72.04\% & 78.56x \\
%     \hline
%     \multirow{3}{*}{MobileNetV2} & \multirow{3}{*}{2.41M} & Baseline & 32 & 75.54\% & 1x \\
%     & & BSQ & 8 & 75.13\% & 6.22x \\
%     & & BWQ-A & 4 & 74.57\% & 18.35x \\
%     \hline
%     \multirow{3}{*}{DenseNet121} & \multirow{3}{*}{7.0M} & Baseline & 32 & 75.99\% & 1x \\
%     & & BSQ & 5 & 75.18\% & 7.26x \\
%     & & BWQ-A & 4 & 75.07\% & 23.65x \\
%     \bottomrule
%   \end{tabular}
%   \label{cifar100}
%   % \vspace{-6pt}
% \end{table}

% \begin{table}
% % \vspace{-6pt}
%   \centering
%   \caption{Model Performance On ImageNet Dataset}
%   % \small
%   \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \multirow{2}{*}{{Model}} & \multirow{1}{*}{{Model}} & \multirow{2}{*}{{Method}} & \multirow{1}{*}{{Act.}} & \multirow{2}{*}{{Acc}} & \multirow{2}{*}{{Comp}} \\
%      & {Size}& & {Prec.} & &  \\
%     % & & & & \\
%     \hline \hline
%     \multirow{3}{*}{ResNet34} & \multirow{3}{*}{21.8M} & Baseline & 32 & 73.55\% & 1x \\
%     & & BSQ & 4 & 72.62\% & 9.48x \\
%     & & BWQ-A & 4 & 72.56\% & 13.55x \\
%     \hline
%     \multirow{3}{*}{DenseNet121} & \multirow{3}{*}{7.0M} & Baseline & 32 & 74.65\% & 1x \\
%     & & BSQ & 5 & 73.70\% & 7.47x \\
%     & & BWQ-A & 4 & 73.68\% & 12.56x \\
%     \bottomrule
%   \end{tabular}
%   \label{imagenet}
%   % \vspace{-6pt}
% \end{table}

% \begin{table*}[t]
%   \centering
%   \caption{Model Performance Comparison.}
%   \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%     \toprule
%     \multirow{3}{*}{{Dataset}} 
%     & \multirow{3}{*}{{Model}} 
%     & \multirow{2}{*}{{\#Param}} 
%     & \multirow{2}{*}{{Baseline Acc}} 
%     & \multicolumn{3}{c|}{BSQ}
%     & \multicolumn{3}{c}{BWQ-A}\\
%     \cline{5-10}
%      &  &  &  &  Act. & Acc & Comp. & Act. & Acc & Comp. \\
%      &  & (M) & (\%) & Prec. & (\%) & ($\times$) & Prec. & (\%) & ($\times$) \\
%     \hline \hline
%     \multirow{6}{*}{CIFAR-10} & ResNet-18 & 11.17   & 95.38  & 4 & 95.38  & 26.05   & 3 & 94.59  & 56.46   \\
%      & ResNet-34 & 21.28   & 95.61  & 4 & 94.66  & 83.86   & 4 & 94.73  & 117.52   \\
%      & VGG16-BN & 33.65   & 92.60  & 3 & 92.45  & 26.59   & 3 & 92.60  & 136.01   \\
%      & VGG19-BN & 38.96   & 92.94  & 3 & 92.84  & 28.15   & 3 & 91.96  & 443.01   \\
%      & ResNet-20 & 0.27   & 92.61  & 3 & 92.16  & 13.76   & 3 & 92.07  & 16.04   \\
%      &  MobileNetV2 & 2.30   & 94.43  & 4 & 94.24  & 5.73   & 3 & 93.54  & 47.34   \\
%     \hline
%     \multirow{6}{*}{CIFAR-100} & ResNet18 & 11.22   & 75.61  & 4 & 76.35  & 6.21   & 4 & 75.31  & 45.97   \\
%      & ResNet34 & 21.33   & 76.41  & 4 & 76.37  & 33.40   & 4 & 76.16  & 63.93   \\
%      & VGG16-BN & 34.02   & 72.93  & 4 & 72.37  & 19.88   & 3 & 72.87  & 50.42   \\
%      & VGG19-BN & 39.33   & 72.94  & 4 & 72.05  & 23.09   & 3 & 72.04  & 78.56   \\
%      &  MobileNetV2 & 2.41   & 75.54  & 8 & 75.13  & 6.22   & 4 & 74.57  & 18.35   \\
%      & DenseNet121 & 7.00   & 75.99  & 5 & 75.18  & 7.26   & 4 & 75.07  & 23.65   \\
%     \hline
%     \multirow{2}{*}{ImageNet} & ResNet34 & 21.80 & 73.55  & 4 & 72.62  & 9.48   & 4 & 72.56  & 13.55   \\
%      & DenseNet121 & 7.98 & 74.65  & 5 & 73.70  & 7.47   & 4 & 73.68  & 12.56   \\

%     \bottomrule
%   \end{tabular}
%   \label{combinedtable}
% \end{table*}

% Due to the high density of ReRAM cells, ReRAM-based accelerators are highly beneficial for edge devices.
% However, to pursue higher representational capabilities, the size of DNN models keeps expanding. 
% For instance, ViT-Huge \cite{dosovitskiy2020image} contains 632M parameters, while the GPT-3 \cite{brown2020language} comprises 175B parameters. 
% It is not a practical solution to scale up the chip size on the edge devices to accommodate these growing DNN models.
% Therefore, efficient model compression techniques are desired.


% On the other hand, several recent works have revealed that 
